Church => Scott = Ptime: an application of resource sensitive realizability

We introduce a variant of linear logic with second order quantifiers and type fixpoints, both restricted to purely linear formulas. The Church encodings of binary words are typed by a standard non-linear type `Church,' while the Scott encodings (purely linear representations of words) are by a linear type `Scott.' We give a characterization of polynomial time functions, which is derived from (Leivant and Marion 93): a function is computable in polynomial time if and only if it can be represented by a term of type Church => Scott. To prove soundness, we employ a resource sensitive realizability technique developed by Hofmann and Dal Lago.

==> eptcsdata.tex <==
\providecommand{\event}{P. Baillot (Ed.): Workshop on Developments in\\
 Implicit Computational complExity (DICE 2010). }
\providecommand{\volume}{23}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{31}
\providecommand{\eid}{3}

